Deformable Temporal Convolutional Networks for Monaural Noisy Reverberant Speech Separation

Speech separation models are used for isolating individual speakers in many speech processing applications. Deep learning models have been shown to lead to state-of-the-art (SOTA) results on a number of speech separation benchmarks. One such class of models known as temporal convolutional networks (TCNs) has shown promising results for speech separation tasks. A limitation of these models is that they have a fixed receptive field (RF). Recent research in speech dereverberation has shown that the optimal RF of a TCN varies with the reverberation characteristics of the speech signal. In this work deformable convolution is proposed as a solution to allow TCN models to have dynamic RFs that can adapt to various reverberation times for reverberant speech separation. The proposed models are capable of achieving an 11.1 dB average scale-invariant signalto-distortion ratio (SISDR) improvement over the input signal on the WHAMR benchmark. A relatively small deformable TCN model of 1.3M parameters is proposed which gives comparable separation performance to larger and more computationally complex models.

==> archive/analysis_backup.tex <==
% Offsets against T60
% \subsection{Offsets vs. T60}
In the following the offsets of each convolutional block for the best performing \ac{DTCN} model $\{X,R\}=\{8,3\}$ are analysed against reverberation time (T60) variation in the WHAMR evaluation set. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fig.~\ref{fig:mutaut60} shows the mean offset values computed in across the each convolutional block and frame index $\ell$ in the aforementioned model for each example in the evaluation set.
% \begin{figure}[!ht]
%     \centering
%     \adjustbox{trim=0cm 0.26cm 0cm 0.23cm,clip}{
%         \includesvg{mean_line_T60_1d.svg}
%     }
%     \caption{Mean values of each offset against reverberation time in T60 for each example in the WHAMR evaluation set. Lines of best fit are plotted in black and Pearson correlation coefficient given on the right for each offset $\tau_p.$}
%     \label{fig:mutaut60}
% \end{figure}
% The outermost kernel offsets, $\tau_1$ and $\tau_3$, have a slight negative correlation with reverberation time. Conversely the middle kernel offset $\tau_2$ has a slight positive correlation with T60.
% Previous work in using \ac{TCN} models for dereverberation tasks \cite{rfield,wdtcn} would suggest that $\tau_1$ and $\tau_3$ should be diverging from one another, i.e.~widening the \ac{RF}, as the reverberation time increases.  This is not observed clearly in Fig.~\ref{fig:mutaut60} but the difference in Pearson correlation coefficients $\rho$ suggests they are actually converging slightly. The middle offset $\tau_2$ is diverging from $\tau_1$ which is widening the \ac{RF} within the kernel however again this is only a very slight effect.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  To simplify notation $\tau_1$ is used in place of $\tau_{\ell,1}$. Fig.~\ref{fig:mutaut60} shows the difference between mean values of the first offset $\tau_1$ and the second and third offsets $\tau_{2:3}$ across every convolutional block and every frame $\ell$ for each example in the evaluation set. The difference between  $\tau_1$ and $\tau_2$ has a weak trend of increasing across the T60 range with a positive correlation coefficient $\rho=0.12$, i.e.~the \ac{RF} between the first two convolutional weights tends to widen as the T60 increases. This is similar to the findings in \cite{rfield,wdtcn}. Contrary to this, the mean difference between $\tau_1$ and $\tau_3$ has a very small negative correlation, i.e.~the \ac{RF} on average decreases to a very small degree as T60 increases. Note the conclusions found in \cite{rfield,wdtcn} only focus on how \acp{RF} respond in much simpler single speaker dereverberation tasks and do not focus on the \ac{RF} between each individual kernel weight as Fig.~\ref{fig:mutaut60} does. In addition $\tau_1$ and $\tau_3$ are constrained to not exceed the \ac{RF} of their none deformable counterparts for a given kernel size and dilation factor as described beneath \eqref{eq:linterpolate}. Relaxing this constraint would possibly lead to different results.
The difference between $\tau_2$ and $\tau_3$ is omitted for brevity but a general trend of convergence between the second and third weights (narrowing \ac{RF} with increasing T60) can be inferred from the other two subplots and correlation coefficients $\rho$. 
\begin{figure}[!h]
    \centering
    \adjustbox{trim=0cm 0.26cm 0cm 0.23cm,clip}{
        \includesvg{delta_mean_line_T60_1d.svg}
    }
    \caption{Differences between the mean value of the first offset $\bar{\tau}_1$ and the second and third offsets $\bar{\tau}_{2:3}$ against reverberation time in T60 for each example in the WHAMR evaluation set. Lines of best fit are plotted in black and Pearson correlation coefficient $\rho$ is given on the right.}
    \label{fig:mutaut60}
\end{figure}


% This is unexpected behaviour and suggests that the optimal configuration of the \ac{RF} of the network maybe more intricately defined than previous results suggesting larger \acp{RF} are better suited to larger reverberation times in data and vice versa for small reverberation times. It is proposed that this could be due to the network performing denoising and separation as well as dereverberation. \Ac{RF} analysis of these sub-tasks similar to \cite{rfield} across different noise types and mixing \acp{SNR} might provide better insight into why the offsets are behaving the way that they are but this is beyond the scope of this work.

% Variance against Model Depth
% \subsection{Variance vs. Model Depth}
% In this section the variances of the offsets at each block in the network are analysed. In \cite{wdtcn} one finding was that the variance of weights used to adapt a TCN model to increasing smaller and larger reverberation times varies increasingly with each additional convolutional blocks. Here a similar analysis is done to demonstrate any redundancy in the lower blocks in the network.

% Fig.~\ref{fig:varanalysis} shows the both the mean standard deviation per block of the offsets $\tau_{p}$ denoted $\sigma_\tau$ as well as the mean standard deviation for each of the $P$ kernel wieght offsets over all blocks for the \ac{DTCN} model with configuration $\{X,R\}=\{8,3\}$. Per block there is more variation around the 10th to 20th block of the network implying this is where the application of deformable convolution over regular convolution is most useful.
% \begin{figure}[!h]
%     \centering
%     \includesvg{variance_analysis.svg}
%     \caption{Mean standard deviation per block for each of 3 kernel weight index per kernel over the entire evaluation set (top) and mean standard deviation for each kernel weight index over all blocks (bottom).}
%     \label{fig:varanalysis}
% \end{figure}

==> whamr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{WHAMR results for \ac{DTCN} models with varying $X$ and $R$ values compared to their corresponding \ac{TCN} configurations.}
\centering
\label{tab:whamr}
\begin{tabular}{|c|c|c|c|cc|cc|cc|cc|cc|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Model} & $X$ & $R$ & {$\mathcal{R}$ (s)} & \textbf{SDR} & \textbf{$\Delta$SDR} & \textbf{SISDR} & \textbf{$\Delta$SISDR} & \textbf{PESQ} & \textbf{$\Delta$PESQ} & \textbf{ESTOI} & \textbf{$\Delta$ESTOI} & \textbf{SRMR} & \textbf{$\Delta$SRMR} \\ \hline
TCN            & 3          & 8          & 0.121                      & 4.75         & 8.24                  & 2.75           & 8.88                    & 1.64          & 0.51                   & 0.46           & 0.22                    & 7.34          & 4.58                   \\
DTCN           & 3          & 8          & 0.121                      & 4.83         & 8.32                  & 2.95           & 9.07                    & 1.69          & 0.54                   & 0.48           & 0.24                    & 7.35          & 4.6                    \\ \hline
TCN            & 4          & 6          & 0.187                      & 4.91         & 8.4                   & 2.98           & 9.1                     & 1.7           & 0.57                   & 0.49           & 0.26                    & 7.88          & 5.12                   \\
DTCN           & 4          & 6          & 0.187                      & 5.31         & 8.8                   & 3.47           & 9.6                     & 1.76          & 0.61                   & 0.53           & 0.29                    & 8.18          & 5.43                   \\ \hline
TCN            & 5          & 5          & 0.316                      & 5.44         & 8.93                  & 3.51           & 9.63                    & 1.79          & 0.65                   & 0.53           & 0.29                    & 8.19          & 5.43                   \\
DTCN           & 5          & 5          & 0.316                      & 5.68         & 9.17                  & 3.88           & 10.0                    & 1.85          & 0.7                    & 0.56           & 0.33                    & 8.52          & 5.77                   \\ \hline
TCN            & 6          & 4          & 0.509                      & 5.44         & 8.93                  & 3.4            & 9.52                    & 1.75          & 0.62                   & 0.51           & 0.27                    & 7.93          & 5.17                   \\
DTCN           & 6          & 4          & 0.509                      & 5.78         & 9.26                  & 3.96           & 10.08                   & 1.85          & 0.7                    & 0.58           & 0.34                    & 8.38          & 5.63                   \\ \hline
TCN            & 8          & 3          & 1.534                      & 5.61         & 9.1                   & 3.64           & 9.77                    & 1.8           & 0.67                   & 0.55           & 0.31                    & 7.85          & 5.09                   \\
DTCN           & 8          & 3          & 1.534                      & 5.84         & 9.33                  & 4.06           & 10.18                   & 1.86          & 0.69                   & 0.59           & 0.35                    & 8.17          & 5.44                   \\ \hline
\end{tabular}
\end{table*}

==> wsj02mix.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\centering
\caption{WSJ0-2Mix results for \ac{DTCN} models with varying $X$ and $R$ values compared to their corresponding \ac{TCN} configurations.}
\label{tab:wsj02mix}
\begin{tabular}{|c|c|c|c|cc|cc|cc|cc|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Model} & $X$ & $R$ & \textbf{$\mathcal{R}$} (s) & \textbf{SDR} & \textbf{$\Delta$SDR} & \textbf{SISDR} & \textbf{$\Delta$SISDR} & \textbf{PESQ} & \textbf{$\Delta$PESQ} & \textbf{ESTOI} & \textbf{$\Delta$ESTOI} \\ \hline
TCN            & 3          & 8          & 0.121                  & 13.93        & 13.78                 & 13.47          & 13.47                   & 2.72          & 1.43                   & 0.85           & 0.37                    \\
DTCN           & 3          & 8          & 0.121                  & 14.19        & 14.04                 & 13.75          & 13.75                   & 2.73          & 1.43                   & 0.86           & 0.38                    \\ \hline
TCN            & 4          & 6          & 0.187                  & 14.4         & 14.25                 & 13.95          & 13.95                   & 2.81          & 1.51                   & 0.86           & 0.38                    \\
DTCN           & 4          & 6          & 0.187                  & 15.05        & 14.9                  & 14.62          & 14.62                   & 2.87          & 1.57                   & 0.88           & 0.4                     \\ \hline
TCN            & 5          & 5          & 0.316                  & 15.03        & 14.87                 & 14.58          & 14.58                   & 2.94          & 1.65                   & 0.88           & 0.39                    \\
DTCN           & 5          & 5          & 0.316                  & 15.52        & 15.37                 & 15.09          & 15.09                   & 2.97          & 1.67                   & 0.89           & 0.4                     \\ \hline
TCN            & 6          & 4          & 0.509                  & 15.1         & 14.95                 & 14.66          & 14.66                   & 2.96          & 1.67                   & 0.88           & 0.4                     \\
DTCN           & 6          & 4          & 0.509                  & 15.84        & 15.69                 & 15.41          & 15.41                   & 3.06          & 1.75                   & 0.9            & 0.41                    \\ \hline
TCN            & 8          & 3          & 1.534                  & 15.86        & 15.71                 & 15.43          & 15.44                   & 3.09          & 1.79                   & 0.9            & 0.41                    \\
DTCN           & 8          & 3          & 1.534                  & 16.02        & 15.87                 & 15.6           & 15.6                    & 3.11          & 1.81                   & 0.9            & 0.42                    \\ \hline
\end{tabular}
\end{table*}
